A simple abstraction of arrays and maps by program translation

We present an approach for the static analysis of programs handling arrays, with a Galois connection between the semantics of the array program and semantics of purely scalar operations. The simplest way to implement it is by automatic, syntactic transformation of the array program into a scalar program followed analysis of the scalar program with any static analysis technique (abstract interpretation, acceleration, predicate abstraction,.. .). The scalars invariants thus obtained are translated back onto the original program as universally quantified array invariants. We illustrate our approach on a variety of examples, leading to the " Dutch flag " algorithm.

==> simplify.tex <==
\section{Simplification of quantifier-free formulas}
\label{sec:simplify}
The output from the backend analysis may be a complicated first-order arithmetic formula, even though an equivalent and much simpler formula exists.
If using \soft{ConcurInterproc}, this is because of the partitioning;\
if using \soft{Flata}, this is due to the way works internally: the transitive closure of a loop body is computed in disjunctive normal form by a form of saturation, and often several of the disjuncts could be coalesced.
Finally, we are interested in equivalence modulo the assumption on the indices; e.g. if $x,y$ is a pair of indices into a $m \times n$ array, we are interested in equivalence modulo $0 \leq x < m \land 0 \leq y < n$.

In this section, we present a procedure \textsc{DNF-simplify} (Algo.~\ref{algo:dnf-simplify}) that takes as input a formula $F$ in first order logic over a decidable theory, an optional ``universe'' quantifier-free formula $U$ over the same theory (if absent, considered to be always true), and outputs a quantifier free $F'$ in disjunctive normal form such that $F \land U \equiv F' \land U$, where $F'$ is expected to be ``small''.
This algorithm is adapted from an quantifier elimination algorithm \cite[\S4.3]{
Monniaux_LPAR08}.

\begin{algorithm}
\caption{Algorithm \textsc{DNF-simplify}}
\label{algo:dnf-simplify}
\begin{algorithmic}
\Require $F$, $U$
\State $\calA \gets \textsc{atoms}(F)$
\State $F' \gets \emptyset$
\While{$F \land U$ satisfiable}
  \State{$m \gets \textsc{model}(F)$}
  \State{$\calP \gets \textsc{generalize}(\textsc{truePredicates}(\calA,m),U \land \neg F)$}
  \State{$F' \gets F' \cup \{ P \}$}
  \State{$F \gets F \land \neg \bigwedge \calP$}
\EndWhile
\end{algorithmic}
\end{algorithm}

Our procedure first collects (subroutine \textsc{atoms}) the atomic formulas $\calA$ from $F$. With respect to arithmetic, for efficiency, $x \leq y$ should be considered as $y \geq x$, and $x = y$ as $x \geq y \land y \geq x$.
For real or rational variables, $x < y$ and $x > y$ are considered the respective negations of $x \geq y$ and $y \geq x$; for integer variables one may encode $x < y$ as $y \geq x+1$.
Then, it solves the satisfiability problem for $F \land U$ using a SMT-solver, terminating if unsatisfiable, otherwise obtaining a model (satisfying assignment) $m$. This model is turned by $\textsc{truePredicates}(\calA,m)$ into the set of all atoms $A \in \calA$ such that $m \models A$ (alternatively, this conjunction may be directly extracted from the SMT-solver). Clearly, the conjunction of all these atoms implies~$F$.

Subroutine $\textsc{generalize}(\calS, G)$ takes as input a set of predicates $\calS$ such that $\bigwedge \calS \land G$ is unsatisfiable, and returns a subset $\calP$ of $\calS$ such that $\bigwedge \calP \land G$ is still unsatisfiable.
One may simply remove each element $P$ from $\calS$ incrementally, as long as $\bigwedge (\calS \setminus \{ P \}) \land G$ is unsatisfiable, and returning the final $\calS$ as $\calP$, which guarantees that $\calP$ is minimal with respect to~$\subseteq$; this is what we implemented.
A more refined approach would be, at each iteration, to replace $\calS$ by an unsatisfiability core for the set of constraints $G \cup (\calS \setminus \{ P \})$.
There exist more approaches to this problem of finding a \emph{minimal unsatisfiable subset} \cite{DBLP:conf/cav/Marques-SilvaJB13}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> style_cheats.tex <==
\renewcommand{\topfraction}{0.9}	% max fraction of floats at top
\renewcommand{\bottomfraction}{0.8}	% max fraction of floats at bottom
    %   Parameters for TEXT pages (not float pages):
\setcounter{topnumber}{2}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{4}     % 2 may work better
\setcounter{dbltopnumber}{2}    % for 2-column pages
\renewcommand{\dbltopfraction}{0.9}	% fit big float above 2-col. text
\renewcommand{\textfraction}{0.07}	% allow minimal text w. figs
    %   Parameters for FLOAT pages (not text pages):
\renewcommand{\floatpagefraction}{0.7}	% require fuller float pages
	% N.B.: floatpagefraction MUST be less than topfraction !!
\renewcommand{\dblfloatpagefraction}{0.7}	% require fuller float pages

\makeatletter
\setlength\textfloatsep{6mm\@plus 1.5\p@ \@minus 4\p@}
\setlength\floatsep{6mm\@plus 1.5\p@ \@minus 4\p@}
\setlength\intextsep{6mm\@plus 1.5\p@ \@minus 4\p@}
\g@addto@macro\normalsize{%
\abovedisplayskip 7.5\p@ \@plus2\p@ \@minus4\p@
\abovedisplayshortskip \z@ \@plus2\p@
\belowdisplayshortskip 3\p@ \@plus2\p@ \@minus2\p@
\belowdisplayskip \abovedisplayskip
}
\g@addto@macro\small{%
\abovedisplayskip 7.5\p@ \@plus2\p@ \@minus4\p@
\abovedisplayshortskip \z@ \@plus2\p@
\belowdisplayshortskip 3\p@ \@plus2\p@ \@minus2\p@
\belowdisplayskip \abovedisplayskip
}
\renewcommand{\paragraph}{%
  \@startsection{paragraph}{4}%
  {\z@}{2.5ex \@plus 0ex \@minus 1ex}{-1em}%
  {\normalfont\normalsize\itshape}%
}
\makeatother

\newcommand{\killspacebetweensectionandlisting}{\vspace{-1.5em}}

